The Fine Classification of Conjunctive Queries and Parameterized Logarithmic Space Complexity

We perform a fundamental investigation of the complexity of conjunctive query evaluation from the perspective of parameterized complexity. We classify sets of boolean conjunctive queries according to the complexity of this problem. Previous work showed that a set of conjunctive queries is fixed-parameter tractable precisely when the set is equivalent to a set of queries having bounded treewidth. We present a fine classification of query sets up to parameterized logarithmic space reduction. We show that, in the bounded treewidth regime, there are three complexity degrees and that the properties that determine the degree of a query set are bounded pathwidth and bounded tree depth. We also engage in a study of the two higher degrees via logarithmic space machine characterizations and complete problems. Our work yields a significantly richer perspective on the complexity of conjunctive queries and, at the same time, suggests new avenues of research in parameterized complexity.

==> fullclassification.tex <==



\begin{theorem}[Classification Theorem]\label{thm:classification}
Let $\fancya$ be a decidable class of structures of bounded arity
such that $\core(\fancya)$ has bounded tree\-width.
\begin{enumerate}
\item If $\core(\fancya)$ has unbounded pathwidth,
then $$\HOMP{\fancya} \equiv_\pl \HOMP{\T^*}.$$

\item If $\core(\fancya)$ has bounded pathwidth and unbounded tree depth,
then $$\HOMP{\fancya} \equiv_\pl \HOMP{\P^*}.$$

\item If $\core(\fancya)$ has bounded tree depth, then 
$$
\HOMP{\fancya}\in\textup{para-L}.$$

\end{enumerate}
\end{theorem}

\begin{remark}\em  If $\fancya$ is assumed to be only computably enumerable instead of decidable, then the theorem stays true 
understanding all mentioned problems in a suitable way as promise
problems. 
If no computability assumption is placed on $\fancya$,
then the theorem stays true in the non-uniform setting of parameterized 
complexity theory (cf.~\cite{downeyfellows}).
\end{remark}


We break the proof into several lemmas. \medskip

%Koalitis and Vardi ~\cite[Lemma~5.2]{koalititsvardicontainment} 
%showed that the canonical query of a structure of {\em treewidth} $w$ is eq%uivalent to a existential first-order sentence that uses only
%$w+1$ {\em variables}; model-checking such sentences can be done in
%poly%omial time~\cite{vardi}. 

To prove statement (3) of Theorem~\ref{thm:classification} we show
that a structure of {\em tree depth} $w$ 
can be characterized, in a sense made precise, by an existential first-order 
sentence of {\em quantifier rank} $w+1$, and that model-checking such sentences can be done in parameterized logarithmic space.  A proof can be found in Section~\ref{sec:fo}.
%This yields statement (3) in Theorem~\ref{thm:classification}.


\begin{lemma}\label{lem:tdinL} Assume $\mathcal A$ is a decidable class of structures of bounded 
arity such that $\core(\fancya)$ has bounded tree depth. Then  $\HOMP{\fancya}\in\textup{para-L}$.
\end{lemma}




%As for an intuition, imagine for each bag an agent responsible for it. 
%The agents pass around some partial homomorphism. 
%Agent $i$ may pass a homomorphism to agent $i+1$ asking her to to ``accept'' or to agent $i-1$ asking her to ``improve''. 
%If an agent receives a partial homomorphism $f$, then $f$ has domain $\dom(f)\subseteq X_i$; if she is asked to accept, she computes
%the (lexicographically) smallest partial homomorphism $g$ with $\dom(g)=X_i$; 
%if she is asked to improve she computes some partial homomorphism $g$ that extends $f\upharpoonright X_{i-1}$ 
%and is bigger than every extension of $f$. If she succeeds in doing this, she asks agent $i+1$ to accept
%$g\upharpoonright X_{i+1}$. Otherwise she asks agent $i-1$ to improve $f\upharpoonright X_{i-1}$. Agent 0 rejects instead oassing something left, 
%and agent $k-1$ accepts instead passing something right.
% Initially, agent 0 is asked to accept the empty map.
%
%
%We need some notation. 
%We can assume that $A_0=\{1,\ldots,|A_0|\}$, that $\preceq$ is the natural order on $A_0$, and that $B=\{1,\ldots,|B|\}$. View 
%a partial function $f$ from $A_0$ to $B$ as a tuple $(b_1,\ldots,b_{|A_0|})\in\{0,\ldots,|B|\}^{|A_0|}$ where $b_i=f(i)$ if $i\in\dom(f)$, and $b_i=0$ otherwise. 
%The partial functions are then ordered lexicographically. Write $X_{-1}:=\emptyset$ and $X_k:=A_0$. 
%A {\em snapshot}  is a triple $(f,i,b)$ where 
%$i<k$ and $f$ is a partial homomorphism from $\rela$ to $\relb$ with $\dom(f)\subseteq X_i$ and $b\in\{0,1\}$. 
%Call $f$ {\em acceptable for} $i$ if there exists a partial homomorphism $g$ with domain $X_i$ that 
%extends $f$. Further, call $f$ {\em improvable for} $i$ if there exists a partial homomorphism $g$ with domain $X_i$ that extends 
%$f\upharpoonright X_{i-1}$ and that is (lexicographically) bigger than 
%all partial functions with domain $X_i$ extending~$f$. 
%
%Our algorithm writes $(\emptyset,0,1)$ on some worktape and simulates the communication above by iterating the following 
%subprocedure $\mathbb A$: 
%
%\begin{center}
%\fbox{
%\begin{minipage}[t]{12cm}
%$\mathbb A(f,i,b)$ \slash \slash \quad $(f,i,b)$ is a snapshot
%\begin{algorithm}
%\im0  \IF\ $i=-1$  \THEN\ reject
%
%\im0 \IF\  $i=k$ \THEN\ accept
%
%\im0 \IF\ $b=1$ \THEN\
%
%\im1 \IF\ $f$ is acceptable for $i$ \THEN\ 
%
%\im2 compute a minimal $g$ witnessing this
%
%\im2 replace $(f,i,b)$ by $(g\upharpoonright X_{i+1},i+1,1)$
%
%\im1 replace $(f,i,b)$ by $(f\upharpoonright X_{i-1},i-1,0)$
%
%\im0 \IF\  $f$ is improvable for $i$ \THEN\ 
%
%\im1 compute a minimal $g$ witnessing this 
%
%\im1 replace $(f,i,b)$ by $(g\upharpoonright X_{i+1},i+1,1)$
%
%\im0 replace $(f,i,b)$ by $(f\upharpoonright X_{i-1},i-1,0)$
%
%
%\end{algorithm}
%\end{minipage}
%}
%\end{center}
%
%To implement lines 5 and 9 test successively all possible witnesses $g:X_i\to B$; note that any such $g$ is given by at most $w'$ many pairs 
%from $A_0\times B$, so in particular can be stored in allowed space $O(\log |B|+\log |A_0|)$. A single snapshot $(f,i,b)$ needs space 
%$O(\log |B|+\log |A_0|+\log k)$ and this is allowed because $\log |A_0|+\log k$ is effectively bounded in the parameter.
%This way, the iteration $$(\emptyset,0,1)=(f_1,i_1,b_1), (f_2,i_2,b_2), (f_3,i_3,b_3),\ldots$$ 
%can be carried out within the allowed space. We show that it eventually stops with the correct answer. 
%
%To prove this we associate with every $(f_j,i_j,b_j)$ appearing in the iteration a tuple $(b_1,\ldots,b_{|A_0|})$ with entries $\le|B|$.
%Initially, the tuple $h_1$ is constantly 0. Assume we already defined $h_j$. If $b_{j+1}=0$, set $h_{j+1}:=h_j$. If 
%$b_{j+1}=1$ (the communication moves right), $\mathbb A$ on $(f_j,i_j,b_j)$ entered line 6 or 10, and in both cases computed some $g$ 
%the line before; in this case $h_{j+1}$ is obtained from $h_j$ replacing for every $a\in\dom(g)= X_{i_j}$ 
%the $a$th entry by $g(a)$.\medskip
%
%\noindent{\em Claims.} For all $j\ge 1$,
%\begin{enumerate}\itemsep=0pt
%\item $h_j$ is equal to or lexicographically smaller than $h_{j+1}$;
%\item every homomorphism from $\mathbf A_0$ to $\relb$ is bigger than $h_j$;
%\item $h_{j+1}\upharpoonright\bigcup_{t\le i_j}X_t$ is a homomorphism from 
%$\big\langle\bigcup_{t\le i_j}X_i \big\rangle^{\rela_0}$ to $\relb$.
%\end{enumerate}
%
%\noindent{\em Proof of the Claims.} ...TBD... claim 1 is problematic.\hfill$\dashv$\medskip
%
%Assume for the sake of contradiction that the iteration is infinite. 
%The sequence $b_1,b_2,\ldots$ cannot be constant for more than $k-1$ steps, so there are
%infinitely many $j$ such that $(b_j,b_{j+1})=(0,1)$. But then $(f_{j+1},i_{j+1},b_{j+1})$ must have been 
%obtained (applying $\mathbb A$ on $(f_j,i_j,b_j)$) 
%according line 10. In this case $h_{j+1}$ is (lexicographically) bigger than $h_j$. With Claim 1 we get a contradiction.
%
%We thus know the iteration eventually accepts or rejects. That this answer is correct follows from Claims~2 and 3.

To prove statements (1) and (2) of Theorem~\ref{thm:classification}
we need to deal with homomorphism problems for classes $\mathcal A$ that are not 
necessarily decidable. Slightly abusing notation, we say $\HOMP{\fancya}\le_\pl\HOMP{\fancya'}$
for arbitrary classes of structures $\mathcal A,\mathcal A'$ if 
there is a implicitly pl-computable {\em partial} function $F$ that is defined on those 
instances $(\rela,\relb)$ of $\HOMP{\fancya}$ with $\rela\in\fancya$ and maps them to
equivalent instances $(\rela',\relb')$ of $\HOMP{\fancya'}$ with $\rela'\in\fancya'$ such 
that $|\rela'|$ is effectively bounded in $|\rela|$.
By saying that a partial function $F$ is implicitly pl-computable with respect to a parameterization $\kappa$ we mean that there are a computable $f:\mathbb N\to\mathbb N$ and a Turing machine that
on those instances $(x,i,b)$ of $\textsc{Bitgraph}(F)$ such that $F$ is defined on $x$, runs in space $O(f(\kappa(x))+\log|x|)$
and answers $(x,b,i)\stackrel{?}{\in} \textsc{Bitgraph}(F)$; on other instances the machine may do whatever it wants.

%To prove statements (1) and (2) of Theorem~\ref{thm:classification}
%we need to deal with homomorphism problems for classes $\mathcal A$ that are not 
%necessarily decidable. The problem $\HOMP{\fancya}$ is understood to have the parameterization that maps a pair of structures 
%to the size of the first structure.
%For arbitrary classes of structures $\mathcal A,\mathcal A'$ we define 
%$\HOMP{\fancya}\le_\pl\HOMP{\fancya'}$
%to mean that there exists an implicitly pl-computable function (with respect to the parameterization specified above) that 
%maps every instance $(\rela,\relb)$ with $\rela\in\fancya$ of $\HOMP{\fancya}$ to an 
%equivalent instance $(\rela',\relb')$ with $\rela'\in\fancya'$ of $\HOMP{\fancya'}$ such 
%that $|\rela'|$ is effectively bounded in $|\rela|$.\medskip

The following lemma takes care of the reductions from left to right in statements (1) and (2) of Theorem~\ref{thm:classification}. 

\begin{lemma}
\label{lemma:tree-decomp-to-tree}
Let $\fancya$ be a class of structures %of bounded arity 
and $\fancyr \subseteq \T$ be a computably enumerable class of trees.
Assume there is $w \in \nats$ such that every structure in $\fancya$ has a tree decomposition of width 
at most $w$ whose tree is contained in~$\fancyr$.
Then, $$\HOMP{\fancya} \le_{\pl} \HOMP{\fancyr^{*}}.$$
\end{lemma}

\begin{proof}
Let $(\rela, \relb)$ with $\rela\in\fancya$ be an instance of $\HOMP{\fancya}$. Enumerating $\mathcal R$, test successively for $\relt\in\mathcal R$ whether there exists a width $\le w$ tree-decomposition $(\relt,(X_t)_{t \in T})$ of $\rela$.
% with $\relt\in\mathcal R$. 
Since $\rela\in\mathcal A$ this test eventually succeeds, and the time needed is effectively bounded in the parameter $|\rela|$.
 With such a tree-decomposition at hand
 produce the instance $(\relt^*, \relb')$ of the problem $\HOMP{\fancyr^*}$ where the structure $\relb'$ is defined as follows. Write $\dom(f)$ for the domain of a partial function $f$; two partial functions $f$ and $g$ are {\em compatible} if they agree on arguments where they are both defined.
\begin{eqnarray*}
B'&:=& \big\{ f\mid f \mbox{ is a partial homomorphism from } \rela \text{ to } \relb
\text{ and } |\dom(f)| \leq w \big\};\\
E^{\relb'}&:=&\big\{ (f, g) \in B' \times B'\mid \text{ $f$ and $g$ are compatible}\big\};\\
C_t^{\relb'} &:=& \big\{ f\in B'\mid \dom(f) = X_t \big\},\quad\text{ for every $t\in T$}.
\end{eqnarray*}
Suppose that $h$ is a homomorphism from $\rela $ to $\relb$.
Then the mapping $h': T \rightarrow B'$ defined by
$h'(t) = h \upharpoonright X_t$ is straightforwardly verified to be a homomorphism from
$\relt^*$ to $\relb'$.

Conversely, let $h'$ be a homomorphism from $\relt^*$ to $\relb'$. Then, $h'(t)$ is a partial homomorphism from $\rela$ to $\relb$ with domain $X_t$. Since $\relt$ is connected the values of $h'$ are pairwise compatible. Hence 
$h:=\bigcup_{t \in T} h'(t)$ is a function from $\bigcup_{t\in T}X_t=A$ to $B$.
To see $h$ is a homomorphism, consider a tuple 
$(a_1, \ldots, a_r) \in R^{\rela}$ for some $r$-ary relation $R$ in the vocabulary of $\rela$. 
Then $\{ a_1, \ldots, a_r \}$ is contained in some bag $X_t$ since it is a clique in the Gaifman graph of $\rela$ (cf.~\cite[Lemma~4]{bodlaendersurvey}). But $h'(t)$ maps this tuple to a tuple in $R^{\relb}$, so
the mapping $h$ does as well.
\end{proof}

For later use we make the following remark concerning the above proof.

\begin{remark}\label{rem:count} \em 
The previous proof associates with a homomorphism $h$ from $\rela $ to $\relb$
the homomorphism $h'$ from $\relt^*$ to $\relb'$ that maps $t$ to $h\upharpoonright X_t$. This 
association $h\mapsto h'$ is injective because every $a \in A$ appears in some bag $X_t$. It is also surjective: 
a homomorphism $h'$ from $\relt^*$ to $\relb'$, is associated with $h:=\bigcup_{t\in T}h'(t)$; the previous proof argued that $h$ is a homomorphism from $\rela$ to $\relb$.
Hence, there is a bijection between 
the set of homomorphisms from $\rela$ to $\relb$ 
and the set of homomorphisms from $\relt^*$ to $\relb'$.
\end{remark}



At the heart of the proof of Theorem~\ref{thm:classification} is the following sequence of reductions, proved in the following subsection.
The appropriately informed reader will recognize  elements from
Grohe's proof~\cite{Grohe07-otherside} as well as from
Marx~\cite[Lemma 5.2]{marx-toc-treewidth}.


\begin{lemma}[Reduction Lemma] \label{lem:redrow}
Let $\fancya$ be a computably enumerable class of structures of bounded arity, 
let $\fancyg$ be the class of Gaifman
graphs of $\core(\fancya)$, and let $\fancym$ be the class of minors of graphs
in $\fancyg$. Then
\begin{eqnarray*}
\HOMP{\fancym^*} 
&\le_{\pl}& \HOMP{\fancyg^*} \\
&\le_{\pl} &\HOMP{\core(\fancya)^*}\\
&\le_{\pl} &\HOMP{\core(\fancya)} \\
&\le_{\pl}& \HOMP{\fancya}.
\end{eqnarray*}
\end{lemma}

With the Reduction Lemma, we can give the proof of the Classification Theorem.\medskip

\begin{proof}[ Proof of Theorem~\ref{thm:classification}]
The reduction from left to right in statements (1) and (2) follow from 
Lemma~\ref{lemma:tree-decomp-to-tree}.
The reductions from right to left follow from the Reduction Lemma~\ref{lem:redrow} via the Excluded Tree Theorem~\ref{thm:rs}~(2)
and the Excluded Path Theorem~\ref{thm:rs}~(3). Statement (3) is proved as Lemma~\ref{lem:tdinL}.
\end{proof}

\subsection{Proof of the Reduction Lemma}

As a consequence of the assumption that $\fancya$ is computably enumerable,
each of the sets $\fancym^*$, $\fancyg^*$, $\core(\fancya)^*$,
and $\core(\fancya)$ are computably enumerable. The statement of the theorem claims the existence of four reductions. The last one from $ \HOMP{\core(\fancya)} $
to $ \HOMP{\fancya}$ is easy to see. We construct the first three in sequence.

\begin{lemma}
\label{lemma:red-minors-to-graphs}
Let $\fancyg$ be a %computably enumerable 
class of graphs which is computable enumerable,
and let $\fancym$ be the class of minors of graphs in~$\fancyg$.
Then $$\HOMP{\fancym^*}  \le_{\pl} \HOMP{\fancyg^*}.$$
\end{lemma}



\begin{proof}
Let $(\relm^*, \relb)$ with $\relm^*\in\fancym^*$ be an instance of the problem $\HOMP{\fancym^*}$. Enumerating $\fancyg$, test successively for $\relg\in\fancyg$ whether $\relm$ is a minor of $\relg$. Since $\relm\in\fancym$ this test eventually succeeds, and then compute a minor map $\mu$ from $\relm$ to $\relg$. 
The time needed is effectively bounded in the parameter $|\relm^*|$. 
The reduction then produces the instance 
$(\relg^*, \relb')$ of $\HOMP{\fancyg^*}$, where $\relb'$ is defined as follows. 
Let $I$ denote the set $\bigcup_{m \in M} \mu(m)$.
\begin{eqnarray*}
B'&:=& (M \times B) \dot\cup \{ \bot \};\\
E^{\relb'}&:=& \big\{ ((m_1, b_1), (m_2, b_2))\mid  [m_1 = m_2 \Rightarrow b_1 = b_2] \mbox{ and }\\
&&\qquad\qquad\qquad\qquad\qquad\qquad [(m_1, m_2) \in E^{\relm} \Rightarrow (b_1, b_2) \in E^{\relb}] \big\}\\
&&\cup\ \big\{(\bot,b')\mid b'\in B' \}\cup \{(b',\bot)\mid b'\in B'\big\};\\
C_v^{\relb'}&:=&\{(m,b)\mid b\in C_m^{\relb}\},\quad\text{ if }m\in M\text{ and }v\in\mu(m);\\
C_v^{\relb'}&:=&\{\bot\},\quad\text{ if }v\notin I.
\end{eqnarray*}

Suppose that $h$ is a homomorphism from
$\relm^*$ to $\relb$.  
Let $h': G \rightarrow B'$ be the map that sends, for each $m \in M$,
the elements in $\mu(m)$ to $(m, h(m))$ and that sends
all elements $v \notin I$ to $\bot$.
Then $h'$ is
a homomorphism from $\relg^*$ to~$\relb'$.

Suppose that $g$ is a homomorphism from $\relg^*$ to $\relb'$.  We show that $g$ is of the form $h'$
for a homomorphism $h$ from $\relm^*$ to $\relb$.
First, by definition of the $C_v^{\relb'}$, it holds that $g(v) = \bot$ for all $v \notin I$.
Next, let $v, w$ be elements of a set $\mu(m)$, with $m \in M$.
The definition of the $C_v^{\relb'}$ ensures that $g(v)$ and $g(w)$ have the form~$(m, \cdot)$. Since $\mu(m)$ is connected, the  definition of $E^{\relb'}$ ensures that $g(v) = g(w)$. Finally, suppose that $(m_1, m_2) \in E^{\relm}$,
let $(m_1, b_1)$ be the image of $\mu(m_1)$ under $g$, and let $(m_2, b_2)$ be the image of $\mu(m_2)$ under~$g$. We claim that $(b_1, b_2) \in E^{\relb}$. But there  exist $v_1 \in \mu(m_1)$ and $v_2 \in \mu(m_2)$ such that $(v_1, v_2) \in E^{\relg}$. We then have $(g(v_1), g(v_2)) \in E^{\relb'}$ and the definition
of $E^{\relb'}$ ensures that $(b_1, b_2) \in E^{\relb}$.
\end{proof}

\begin{lemma}
\label{lemma:red-graphs-to-structures}
Let $\fancya$ be a computably enumerable class of structures of bounded arity, 
and let $\fancyg$ be the class of Gaifman graphs of~$\fancya$. Then $$\HOMP{\fancyg^*}  \le_{\pl} \HOMP{\fancya^*}.$$
\end{lemma}

\begin{proof}
Let the pair $(\relg^*, \relb)$ with $\relg\in \fancyg$ be an instance of $\HOMP{\fancyg^*}$. Similarly as seen in the previous proof, one can compute from $\relg$ a structure $\rela\in\fancya$ whose Gaifman graph is $\relg$.
The reduction produces the instance $(\rela^*, \relb')$ of
$\HOMP{\fancya^*}$, where $\relb'$ is defined as follows.
\begin{eqnarray*}\itemsep=0pt
B'&:=&B;\\
C_a^{\relb'}&:=&C_a^{\relb},\quad \text{ for every } a\in A;\\
R^{\relb'}&:=&\{(b_1,\ldots,b_r)\mid\{b_1\ldots,b_r\}\text{ is a clique in }(B,E^{\relb})\},
\end{eqnarray*}
for every $r$-ary symbol $R$ from the vocabulary of $\rela$. It is straightforward to verify that a function
$h: A \rightarrow B$ is a homomorphism from $\relg$ to $\relb$ if and only if
it is a homomorphism from $\rela$ to $\relb'$.
\end{proof}

Recall that the {\em direct product} $\rela\times\relb$ of two $\tau$-structures $\rela$ and~$\relb$ has
universe $A\times B$ and interprets a relation symbol $R\in\tau$ by $\{((a_1,b_1),\ldots,(a_{\ar(R)},b_{\ar(R)}))\mid \bar a\in R^\rela,\bar b\in R^\relb\}$.

\begin{lemma}
\label{lemma:reduction-constants-cores}
Let $\fancya$ be a class of structures.
Then $$\HOMP{\core(\fancya)^*} \le_{\pl} \HOMP{\core(\fancya)}.$$
\end{lemma}

\begin{proof} 
Let $(\reld^*, \relb)$ with $\reld\in\core(\fancya)$ be an instance of $\HOMP{\core(\fancya)^*}$.
Let $\relb_*$ be the restriction of $\relb$ to the vocabulary of $\reld$.
The reduction produces the instance $(\reld, \relb')$
of the problem $\HOMP{\core(\fancya))}$, where 
$$
\relb':=\big\langle \big\{ (d, b) \in D \times B\mid b \in C_{d}^{\relb}  \big\}  \big\rangle^{\reld \times \relb_*}.
$$ 

Suppose that $h$ is a homomorphism from $\reld^*$ to $\relb$.
Then, the mapping $h': D \rightarrow B'$ defined by
$h'(d) = (d, h(d))$ is straightforwardly verified to be a homomorphism
from $\reld$ to $\relb'$.

Suppose that $g$ is a homomorphism from $\reld$ to $\relb'$. Write $\pi_1$ and $\pi_2$ for the projections that map a pair to its first and second component respectively.
The composition $(\pi_1 \circ g)$ is a homomorphism from $\reld$ to itself; since $\reld$ is a core,
$(\pi_1 \circ g)$ is bijective.  Hence, there exists a natural $m \geq 1$ such that
$(\pi_1 \circ g)^m$ is the identity  on~$D$. Define $h$ as 
$g \circ (\pi_1 \circ g)^{m-1} $. Clearly, $h$ is a homomorphism from 
$\reld$ to $\relb'$, so $\pi_2 \circ h$ is a homomorphism from 
$\reld$ to $\relb_*$.  We claim that $\pi_2 \circ h$ is also a homomorphism from $\reld^*$ to~$\relb$.
Observe that $\pi_1 \circ h$ is the identity on $D$. In other words, for every $d\in D$ there is $b_d \in B$ such that
$h(d)=(d, b_d)$. By definition of $\relb'$ we get $b_d \in C_d^{\relb}$,
establishing the claim.
\end{proof}

Observe that the map $h'$ constructed in the above proof is an embedding. Hence
we have the following corollary that we note explicitly for later use.

\begin{corollary}\label{cor:coreemb}
Let $\fancya$ be a class of structures.
Then $$
\HOMP{\core(\fancya)^*} \le_{\pl} \EMP{\core(\fancya)}.
$$
\end{corollary}

\subsection{Bounded tree depth and $\textup{para-L}$}\label{sec:fo}


Let $\tau$ be a vocabulary. {\em First-order $\tau$-formulas} are built from {\em atoms} $R\bar x, x=x$ by Boolean 
combinations and existential and universal quantification. Here, $\bar x$ is a tuple of variables of length matching the arity of $R$. 
We write $\varphi(\bar x)$ for a (first-order) $\tau$-for\-mula~$\varphi$
to indicate that the free 
variables in $\varphi$ are among the components of $\bar x$. The {\em quantifier rank} $\qr(\varphi)$ of a formula $\varphi$
is defined as follows: 
\begin{itemize}\itemsep=0pt
\item[] $\qr(\varphi)=0$ \quad for atoms $\varphi$; 
\item[] $\qr(\neg\varphi)=\qr(\varphi)$; 
\item[] $\qr(\varphi\wedge\psi)=\qr(\varphi\vee\psi)=\max\{\qr(\varphi),\qr(\psi)\}$; 
\item[] $\qr(\exists x\varphi)=\qr(\forall x\varphi)=1+\qr(\varphi)$.
\end{itemize}


The following is standard, but we could not find a reference, so include the simple proof for completeness.

\begin{lemma}\label{lem:mcfo} The parameterized problem
%
\npprob{$p$-MC(FO)}{\em A structure $\rela$, a first-order sentence $\varphi$}
{$|\varphi|$}{$\rela\models\varphi$ ?}
can be decided in space  $O(|\varphi|\cdot\log|\varphi|+(\qr(\varphi)+\ar(\varphi))\cdot\log |A|)$, where 
$\qr(\varphi)$ is the quantifier rank of $\varphi$ and 
$\ar(\varphi)$ is the maximal arity over all relation symbols in $\varphi$
\end{lemma}



\begin{proof} We give an algorithm expecting inputs $(\rela,\varphi,\alpha)$ where 
$\varphi$ is a formula and 
$\alpha$ is an assignment for $\varphi$ in $\rela$, that is, a map from a superset of the free variables of $\varphi$ into $A$. The algorithm determines whether $\alpha$ satisfies $\varphi$ in $\rela$. It executes a depth-first recursion as follows. 

If $\varphi$ is an atom $R\bar y$ the algorithm writes 
the tuple $\alpha(\bar y)\in A^{\ar(R)}$ on the worktape and checks whether it is contained in $R^\rela$ by scanning the input; it then erases the tuple and returns the bit corresponding to the answer obtained. 

If $\varphi=(\psi\wedge\chi)$, the algorithm recurses on $\psi$ (with the same assignment); 
upon completing the recursion it erases all space used in it, stores a bit for the answer obtained, and then recurses on $\chi$;
upon completion it erases the space used in it and returns the minimum of the bit obtained and the stored bit.
The cases $\varphi=(\psi\vee\chi)$ and $\varphi=\neg\psi$ are similar.

If $\varphi(\bar x)=\exists y\psi(\bar x,y)$ the algorithm loops through $b\in A$ and recurses on $\psi$ with assignment $\alpha$ 
extended by mapping $y$ to $b$; 
it maintains a bit which is intially 0 and updates it
after each loop to the maximum of the bit obtained in the loop; after each loop it erases the space used in in it.
Upon completing the loop it returns this bit, and restricts the assignment back to its old domain without~$y$.
The case $\varphi(\bar x)=\forall y\psi(\bar x,y)$ is similar.

When started on a sentence $\varphi$ and the empty assignment, all assignments $\alpha$ occuring in the recursion have cardinality $\le \qr(\varphi)$, so can be stored in space $O(\qr(\varphi)\cdot(\log|\varphi|+\log|A|))$. Each recursive step adds space $O(\log|\varphi|)$ to remember
 the (position of) the current subformula plus one bit 
 plus $O(\log |A|)$ 
for the loop on $b\in A$ in the quantifier case and plus $O(\ar(\varphi)\cdot\log |A|)$ in the atomic case.
From these considerations it is routine to verify the claimed upper bound on space.
%
%Each recursive step adds space $O(\log|\varphi|)$ to remember the (position of) the subformula $\psi$ plus one bit plus $O(\log |A|)$ 
%for the loop on $b\in A$ in the quantifier case and plus $O(\ar(\varphi)\cdot\log |A|)$ in the atomic case. The assignments $\alpha$ occuring in the recursion 
%all have cardinality $w\le \qr(\varphi)$, so need space $O(w(\log|\varphi|+\log|A|))$ to be stored. 
\end{proof}


The {\em canonical conjunction} of a structure $\rela$ is a quantifier-free conjunction in the variables $x_a$ for $a\in A$; namely, 
for every relation symbol $R$ of $\rela$ and every  $(a_1,\ldots, a_{\ar(R)})\in R^\rela$ it contains the conjunct
$Rx_{a_1}\cdots x_{a_{\ar(R)}}$. It is easy to see that the canonical
conjunction of $\rela$ 
is satisfiable in a
structure $\relb$ if and only if there is an homomorphism from $\rela$ to~$\relb$.


\begin{proof}[Proof of Lemma~\ref{lem:tdinL}] 
Choose $w\in\mathbb N$ such that $\td(\core(\rela))\le w$ for all $\rela\in\fancya$. 
Given a structure $\rela$ we compute a sentence $\varphi_\rela$ of quantifier rank at most $w+1$ such that for all structures $\relb$, the sentence $\varphi_\rela$ is true in $\relb$ if and only if there
is a homomorphism from $\rela$ to $\relb$. 
This is enough by Lemma~\ref{lem:mcfo}.

Given $\rela$ we check $\rela\in\fancya$ running some decision procedure for $\fancya$. If
 $\mathbf A\notin\fancya$ we let $\varphi_\rela:=\exists x\ \neg x=x$. 
If $\rela\in\fancya$, compute the core $\mathbf A_0$ of $\mathbf A$ and compute for every connected component $C$ of the Gaifman graph of $\rela_0$ some 
rooted tree $\relt$ with vertices $T=C$ and height at most $w$ such that every edge of the 
Gaifman graph of $\langle C\rangle^{\rela_0}$ is in the closure of $\relt$.

Consider a component $C$ and let $\relt$ be the rooted tree computed for $C$.
For $c\in C=T$ we compute the following first-order formula $\varphi_c$. We use variables $x_c$ for $c\in C=T$. 
If $c$ is a leaf of $\relt$, let $\varphi_c$ be the canonical conjunction of $\langle P_c\rangle^{\rela_0}$ where $P_c$ is 
the path  in $\relt$ leading from the root $r$ of $\relt$ to $c$.
For an inner vertex $c$ define
$$\textstyle
\varphi_c:=\bigwedge_{d} \exists x_d\ \varphi_d,
$$ 
where $d$ ranges over the successors of $c$. 
The following claims are straightforwardly verified by induction along the recursive definition of the $\varphi_c$s.

\medskip

\noindent{\em Claims.} For every $c\in C$:
\begin{enumerate}\itemsep=0pt
 \item the quantifier rank of $\varphi_c$ equals the height of the subtree of $\relt$ rooted at $c$;
\item the free variables of $\varphi_c$ are $\{x_d\mid d\in P_c\}$;
\item $\varphi_c$ is satisfiable in $\relb$ if and only if so is the canonical conjunction of 
$\langle C(c)\rangle^{\rela_0}$ where $C(c)$ contains $P_c$ and the vertices in the subtree rooted at $c$.
\end{enumerate}

Letting $r$ range over the roots of the trees $\relt$ chosen for the connected components $C$ of $\rela_0$, we set
$$\textstyle
\varphi_\rela:=\bigwedge_r\exists x_r\varphi_r.
$$ 
By Claim 2 this is a sentence and by Claim 1 it has quantifier rank at most $w+1$. It is true in $\relb$ if and only if every 
$\exists x_r\varphi_r$ is true in $\relb$, and by Claim 3 this holds  if and 
only if the canonical conjunction of 
$\langle C(r)\rangle^{\rela_0}$ is satisfiable in $\relb$ for every 
connected component $C$. Noting $C(r)=C$, this means
that every $\langle C\rangle^{\rela_0}$ maps 
homomorphically to $\relb$, and this means that $\rela_0$ maps homomorphically to $\relb$. Recalling that
$\rela_0$ is the core of $\rela$, we see that this is equivalent to $\rela$ mapping homomorphically to $\relb$.
 \end{proof} 



Define a
$\{ \wedge, \exists \}$-sentence
to be a first-order sentence built from atoms,
conjunction,
and existential quantification.
The previous proof revealed that, given a structure $\rela$
with 
$\td(\core(\rela))\le w$,
there exists a 
$\{ \wedge, \exists \}$-sentence $\phi$ 
of quantifier rank at most $w + 1$
that \emph{corresponds} to $\rela$ in that,
for all structures $\relb$,
the sentence $\phi$ is true on $\relb$ 
if and only if there is a homomorphism
from $\rela$ to $\relb$.
We show that the existence of such a sentence in fact characterizes
tree depth, in the following precise sense.

\begin{theorem}
Let $w \geq 0$, and let $\rela$ be a structure.
It holds that $\td(\core(\rela)) \le w$
if and only if
there exists a $\{ \wedge, \exists \}$-sentence $\phi$
that corresponds to $\rela$ with $\qr(\phi) \leq w + 1$.
\end{theorem}

\begin{proof}
The forward direction follows from the previous proof.
For the backward direction, let $\phi$ be a sentence of the described
type.
We may assume that no variable is quantified twice in $\phi$
and that no equality of variables appears in $\phi$,
by renaming variables and replacing equalities of the form $v = v$
with the empty conjunction.
Let $\phi_p$ be the prenex sentence where all variables that are
existentially quantified in $\phi$ are existentially quantified in
$\phi_p$,
and the quantifier-free part of $\phi_p$ is the conjunction of all 
atoms appearing in $\phi$.
Let $\relc$ be a structure whose canonical conjunction is 
the quantifier-free part of $\phi_p$.
Clearly, $\phi_p$ and the original $\phi$ are logically equivalent;
it follows that $\relc$ and $\rela$ are 
homomorphically equivalent~\cite{ChandraMerlin77-optimal}.
It thus suffices to show that $\td(\relc) \leq w$.

View the sentence $\phi$ as a directed graph, and
define an acyclic directed graph $D$ on the variables of $\phi$
where the directed edge $(v, v')$ is present if and only if
the node for $\exists v$ is the first node with quantification
occurring above the node for $\exists v'$.
Let $\alpha$ be an arbitrary atom from $\phi_p$
(equivalently, from $\phi$).
Since $\phi$ is a sentence, if one traverses $\phi$ starting from 
the root and moving to $\alpha$,
one will pass a node $\exists v$ for each variable $v$ of
$\alpha$.
Let $v_1, \ldots, v_k$ be the variables of $\alpha$ in the order
encountered by such a traversal.  
The edges $(v_1, v_2), (v_2, v_3), \ldots, (v_{k-1}, v_k)$ are in 
the transitive closure of $D$, and hence in the closure of 
the graph underlying $D$ (where a node is a root in the graph 
iff it is parentless in $D$).
Since $\qr(\phi) \leq w + 1$, each directed path in $D$ has length
less than or equal to $w$, and so 
the graph underlying $D$ witnesses that $\td(\relc) \leq w$.
\end{proof}


We now show the following result on the embedding problem.

\begin{theorem}\label{theo:embtd}
 Assume $\mathcal A$ is a decidable class of structures of bounded 
arity and  bounded tree depth. Then  $\EMP{\fancya}\in\textup{para-L}.$
\end{theorem}

The proof of this result uses color coding methods, more precisely, it relies on the following lemma (see~\cite[p.349]{flumgrohe}).

\begin{lemma}\label{lem:hash} For every sufficiently large $n$, it holds that for all $k\in\mathbb N$ and 
for every $k$-element subset $X$ of $[n]$, 
there exists a prime $p<k^2\log n$ and $q<p$ such that the function 
$h_{p,q}:[n]\to\{0,\ldots,k^2-1\}$ given by 
$$
h_{p,q}(m):= (q\cdot m \textup{ mod } p) \textup{ mod } k^2
$$
 is injective on $X$. 
\end{lemma}

For later use we give the main step in the proof of Theorem~\ref{theo:embtd} as a separate lemma. Call a structure {\em connected} if 
its Gaifman graph is connected.


\begin{lemma}\label{lem:connected}
For every decidable class of connected structures $\fancya$ we have $$\EMP{\fancya}\le_\pl\HOMP{\fancya^*}.$$
\end{lemma}

\begin{proof}
 Map an instance $(\rela,\relb)$ to $(\rela^*,\relb_*)$ where $\relb_*$ is defined as follows. We assume that $B=[|B|]$ and $A=[|A|]$. Let $F$ be the set
$$
\big\{g\circ h_{p,q}\mid  g:\{0,\ldots,|A|^2-1\}\to A \text{ and }q<p<|A|^2\log|B|\big\}.
$$
Here, $h_{p,q}:[|B|]\to\{0,\ldots,|A|^2-1\}$ is the function from Lemma~\ref{lem:hash} (for $n:=|B|$ and $k:=|A|$).
For $f\in F$, let $\relb_f$ be the expansion of $\relb$ that interprets every $C_a,a\in A,$ by $f^{-1}(a)\subseteq B$ and define $\relb_*$ as the disjoint union of the structures $\relb_f$. 
We verify 
$$
(\rela,\relb)\in\EMP{\fancya}\Longleftrightarrow (\rela^*,\relb_*)\in\HOMP{\fancya^*}.
$$
Note that the sets $C^{\relb_*}_a, a\in A$,  are pairwise disjoint, so every homomorphism from $\rela^*$ to $\relb_*$ is an embedding. And because $\rela^*$ is connected, it is an embedding into (the copy of) some $\relb_f$, so it corresponds to an embedding from $\rela$ into~$\relb$.
 Conversely, assume $e$ is an embedding of $\rela$ into $\relb$. 
By Lemma~\ref{lem:hash} there are $p,q$ with $q<p<|A|^2\log |B|$ such that $h_{p,q}$ is 
injective on the image of $e$. Then there exists $g:\{0,\ldots,|A|^2-1\}\to A$ 
such that $g\circ h_{p,q}\circ e$ is 
the identity on $A$. Then $f:=g\circ h_{p,q}\in F$ and $e$ is an embedding of $\rela^*$ into~$\relb_{f}$ and hence into $\relb_*$. 
\end{proof}

This lemma together with Corollary~\ref{cor:coreemb} implies:

\begin{corollary}\label{cor:embhom}
Let $\fancya$ be a decidable class of connected cores. Then $$\HOMP{\fancya^*}\equiv_\pl\EMP{\fancya}.$$
\end{corollary}


\begin{proof}[Proof of Theorem~\ref{theo:embtd}] Let $\fancya$ accord the assumption. 

\medskip

\noindent{\em Claim.} There exists a decidable class of connected structures $\fancya'$ of
 bounded tree depth such that $\EMP{\fancya}\le_\pl\EMP{\fancya'}$.\medskip

Note $\EMP{\fancya'}\le_\pl\HOMP{(\fancya')^*}$ by the previous lemma and $\HOMP{(\fancya')^*}\in\textup{para-L}$ by Lemma~\ref{lem:tdinL}. 
We are thus left to prove the claim.


 Assume $\fancya$ has tree depth at most $d$ and let $E$ be a binary relation symbol not occuring in the vocabulary 
of any $\rela\in\fancya$. Fix a computable function that maps every $\rela\in\fancya$ to a family
of height $\le d$ rooted trees $(\relt_C)_C$ with $\relt_C=(C,E^{\relt_C},\textit{root}^{\relt_C})$ where $C$
ranges over the connected components of the 
Gaifman graph $\relg(\rela)$ of $\rela$, and such that $\langle C\rangle^{\relg(\rela)}$ is a subgraph of the closure of $\relt_C$. 
Define $\rela'$ to be the expansion of $\rela$ interpreting $E$ by $\bigcup_CE^{\relt_C}\cup E'$ where $E'$ is defined as follows. It
contains edges between the root of $\relt_{C_0}$ and the roots of the other $\relt_{C}$ 
where $C_0$ is the lexicographically minimal component (according to the encoding of $\rela$).
Then $\rela'$ is connected and has tree depth at most $d+1$. 
Clearly, $\fancya':=\{\rela'\mid\rela\in\fancya\}$ is decidable. The map $(\rela,\relb)\mapsto(\rela',\relb')$, where $\relb'$ 
is the expansion of $\relb$ interpreting $E$ by $B^2$, is a pl-reduction from $\EMP{\fancya}$ to $\EMP{\fancya'}$.
\end{proof}










